Analysis of the Effect of Dependency Information on Predicate-Argument Structure Analysis and Zero Anaphora Resolution

This paper investigates and analyzes the effect of dependency information on predicate-argument structure analysis (PASA) and zero anaphora resolution (ZAR) for Japanese, and shows that a straightforward approach of PASA and ZAR works effectively even if dependency information was not available. We constructed an analyzer that directly predicts relationships of predicates and arguments with their semantic roles from a POS-tagged corpus. The features of the system are designed to compensate for the absence of syntactic information by using features used in dependency parsing as a reference. We also constructed analyzers that use the oracle dependency and the real dependency parsing results, and compared with the system that does not use any syntactic information to verify that the improvement provided by dependencies is not crucial.

==> table_dep_n20_2.tex <==
\begin{table}[t]
\tbl{\label{Table:Dependency-E20}{\sf PWPASA + Dep.(20\% errors)}: Results of the analyzer that uses the noisy dependency information (includes 20\% simulated errors).}{
%\begin{center}
%\scriptsize{
\begin{tabular}{|l|l|@{\onesp}r@{\onesp}|@{\onesp}r@{\onesp}|@{\onesp}r@{\onesp}|}
\hline
Role type & Category & P & R & F\\
\hline
\hline
\multirow{8}{*}{{\it ga} (nom.)} & \multirow{2}{*}{Depend} & 88.21 & 63.49 & 73.84 \\
& & (10033/11374) & (10033/15803) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 54.33 & 19.04 & 28.20 \\
& & (1505/2770) & (1505/7906) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 23.78 & 5.97 & 9.54 \\
& & (322/1354) & (322/5396) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 76.53 & 40.75 & 53.18 \\
& & (11860/15498) & (11860/29105) & \\
\hline
\multirow{8}{*}{{\it wo} (acc.)} & \multirow{2}{*}{Depend} & 97.22 & 82.42 & 89.21 \\
& & (8721/8970) & (8721/10581) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 62.12 & 18.71 & 28.76 \\
& & (264/425) & (264/1411) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 33.33 & 1.90 & 3.59 \\
& & (16/48) & (16/843) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 95.32 & 70.13 & 80.81 \\
& & (9001/9443) & (9001/12835) & \\
\hline
\multirow{8}{*}{{\it ni} (dat.)} & \multirow{2}{*}{Depend} & 96.80 & 83.40 & 89.60 \\
& & (2206/2279) & (2206/2645) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 40.76 & 17.65 & 24.63 \\
& & (75/184) & (75/425) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 16.28 & 2.71 & 4.65 \\
& & (7/43) & (7/258) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 91.30 & 68.75 & 78.44 \\
& & (2288/2506) & (2288/3328) & \\
\hline
\multirow{8}{*}{ALL} & \multirow{2}{*}{Depend} & 92.65 & 72.22 & 81.17 \\
& & (20960/22623) & (20960/29029) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 54.57 & 18.93 & 28.11 \\
& & (1844/3379) & (1844/9742) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 23.88 & 5.31 & 8.69 \\
& & (345/1445) & (345/6497) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 84.34 & 51.14 & 63.67 \\
& & (23149/27447) & (23149/45268) & \\
\hline
\end{tabular}
}
%\end{center}
\end{table}


==> table_indep.tex <==
\begin{table}[t]
\tbl{\label{Table:Proposed-indep}{\sf PWPASA - Lang. F.}: Results of the PWPASA analyzer that does not use the dependency information and the language dependent features.}{
%\begin{center}
%\scriptsize{
\begin{tabular}{|l|l|@{\onesp}r@{\onesp}|@{\onesp}r@{\onesp}|@{\onesp}r@{\onesp}|}
\hline
Role type & Category & P & R & F\\
\hline
\hline
\multirow{8}{*}{{\it ga} (nom.)} & \multirow{2}{*}{Depend} & 88.96 & 57.84 & 70.10 \\
& & (9140/10274) & (9140/15803) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 50.85 & 24.48 & 33.05 \\
& & (1935/3805) & (1935/7906) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 23.42 & 5.69 & 9.15 \\
& & (307/1311) & (307/5396) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 73.96 & 39.11 & 51.16 \\
& & (11382/15390) & (11382/29105) & \\
\hline
\multirow{8}{*}{{\it wo} (acc.)} & \multirow{2}{*}{Depend} & 97.10 & 83.14 & 89.58 \\
& & (8797/9060) & (8797/10581) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 56.41 & 22.75 & 32.42 \\
& & (321/569) & (321/1411) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 35.00 & 1.66 & 3.17 \\
& & (14/40) & (14/843) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 94.45 & 71.15 & 81.16 \\
& & (9132/9669) & (9132/12835) & \\
\hline
\multirow{8}{*}{{\it ni} (dat.)} & \multirow{2}{*}{Depend} & 95.01 & 81.36 & 87.66 \\
& & (2152/2265) & (2152/2645) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 39.39 & 18.35 & 25.04 \\
& & (78/198) & (78/425) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 13.79 & 1.54 & 2.79 \\
& & (4/29) & (4/258) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 89.65 & 67.13 & 76.77 \\
& & (2234/2492) & (2234/3328) & \\
\hline
\multirow{8}{*}{ALL} & \multirow{2}{*}{Depend} & 93.01 & 69.20 & 79.36 \\
& & (20089/21599) & (20089/29029) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it intra})} & 51.05 & 23.96 & 32.61 \\
& & (2334/4572) & (2334/9742) & \\
\cline{2-5}
& \multirow{2}{*}{Zero~({\it inter})} & 23.55 & 5.00 & 8.25 \\
& & (325/1380) & (325/6497) & \\
\cline{2-5}
& \multirow{2}{*}{ALL} & 82.57 & 50.25 & 62.48 \\
& & (22748/27551) & (22748/45268) & \\
\hline
\end{tabular}
}
%\end{center}
\end{table}

